Towards a Unified Multimodal Reasoning Framework

Recent advancements in deep learning have led to the development of powerful language models (LMs) that excel in various tasks. Despite these achievements, there is still room for improvement, particularly in enhancing reasoning abilities and incorporating multimodal data. This report investigates the potential impact of combining Chain-of-Thought (CoT) reasoning and Visual Question Answering (VQA) techniques to improve LM's accuracy in solving multiple-choice questions. By employing TextVQA and ScienceQA datasets, we assessed the effectiveness of three text embedding methods and three visual embedding approaches. Our experiments aimed to fill the gap in current research by investigating the combined impact of CoT and VQA, contributing to the understanding of how these techniques can improve the reasoning capabilities of state-of-the-art models like GPT-4. Results from our experiments demonstrated the potential of these approaches in enhancing LM's reasoning and question-answering capabilities, providing insights for further research and development in the field, and paving the way for more accurate and reliable AI systems that can handle complex reasoning tasks across multiple modalities.

==> contributions.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{|l|p{15em}|p{10cm}|}
\hline
Student Name & Contributed Aspects & Details \\
\hline\hline
Abhinav Arun & ViLT,DeTR, Image Captioning, Experimental designs on T5 Models & Fine-tuned ViLT for question answering on Science QA dataset by creating custom config vocabularies and annotations. Generated Image captions using ViT-GPT2 and worked on its integration in the T5 finetuning scripts for Science QA. Designed training scripts and tested various hypotheses using experiments on T5 models. \\ 
Dipendra Singh Mal & T5 Finetuning Script. Training and Evaluation of T5 models & Built the script to finetune and run experiments on T5 model focusing on textual data from ScienceQA. fine-tuned and evaluated T5 models for generating answers, explanation and lecture.\\
Mehul Soni & DeTR,ViLT, Image Captioning , T5 models scripts and exploration & Generated vision features using DeTR, helped in the integration of image captions in T5 models, Developed training scripts for T5 model on ScienceQA and TextVQA dataset. Explored various experiments on the Science QA dataset. \\ 
Tomohiro Sawada & Training baseline models. Draft writing. & Trained the baseline models (RoBERTa and DistilBERT) on the ScienceQA dataset. Contributed to writing drafts of the final paper.\\
\hline
\end{tabular}
\end{center}
\caption{Contributions of team members.}
\label{tab:contributions}
\end{table*}
